Breaking the Curse of Multiagency: Provably Efficient Decentralized Multi-Agent RL with Function Approximation

A unique challenge in Multi-Agent Reinforcement Learning (MARL) is the curse of multiagency, where the description length of the game as well as the complexity of many existing learning algorithms scale exponentially with the number of agents. While recent works successfully address this challenge under the model of tabular Markov Games, their mechanisms critically rely on the number of states being finite and small, and do not extend to practical scenarios with enormous state spaces where function approximation must be used to approximate value functions or policies. This paper presents the first line of MARL algorithms that provably resolve the curse of multiagency under function approximation. We design a new decentralized algorithm -- V-Learning with Policy Replay, which gives the first polynomial sample complexity results for learning approximate Coarse Correlated Equilibria (CCEs) of Markov Games under decentralized linear function approximation. Our algorithm always outputs Markov CCEs, and achieves an optimal rate of $\widetilde{\mathcal{O}}(\epsilon^{-2})$ for finding $\epsilon$-optimal solutions. Also, when restricted to the tabular case, our result improves over the current best decentralized result $\widetilde{\mathcal{O}}(\epsilon^{-3})$ for finding Markov CCEs. We further present an alternative algorithm -- Decentralized Optimistic Policy Mirror Descent, which finds policy-class-restricted CCEs using a polynomial number of samples. In exchange for learning a weaker version of CCEs, this algorithm applies to a wider range of problems under generic function approximation, such as linear quadratic games and MARL problems with low ''marginal'' Eluder dimension.

==> Sections/linear_assumption.tex <==
\section{Independent linear function approximation}
\label{sec:linear-assumption}
\subsection{Assumption for Independent Linear Function Approximation}

We want an assumption that meets the three following criteria:
\begin{itemize}
    \item Does not trivialize the problem (imply essentially tabular or essentially single-player);
    \item Contains the Linear MDP + Tabular MG example;
    \item Enables a linear SPoCMAR-type algorithm.
\end{itemize}

Consider the following assumptions.


\begin{assumption}[All $\pi$ V-V]
For any $(i,h)\in[m]\times[H]$ and function $\oV_{i,h+1}$ and any policy $\pi$, we have 
\begin{align*}
\DD_\pi\brac{r_{i,h} + \P_h\oV_{i,h+1}}(s) = \phi(s)^\top \theta^{h,\pi,\oV}
\end{align*}
for some $\theta^{h,\pi,\oV}$.
\end{assumption}

\begin{assumption}[All $\pi$ Q-V]
For any $(i,h)\in[m]\times[H]$ and function $\oV_{i,h+1}$ and any policy $\pi_{-i}$ of other players, we have 
\begin{align*}
\DD_{\delta_a\times \pi_{-i}}\brac{r_{i,h} + \P_h\oV_{i,h+1}}(s) = \phi_i(s,a)^\top \theta^{h,\pi_{-i},\oV}
\end{align*}
for some $\theta^{h,\pi,\oV}$.
\end{assumption}

\begin{assumption}[Greedy $\pi$ V-V]
For any $(i,h)\in[m]\times[H]$ and function $\oV_{i,h+1}$ and any policy $\pi\in \Pi^{lin}$, we have 
\begin{align*}
\DD_\pi\brac{r_{i,h} + \P_h\oV_{i,h+1}}(s) = \phi(s)^\top \theta^{h,\pi,\oV}
\end{align*}
for some $\theta^{h,\pi,\oV}$.
\[\Pi^{lin}:=\left\{\pi_i(\cdot|s) = \arg\max_a\left(\phi(s)^\top w^{a,i}\right)\right\}\]
\end{assumption}

\begin{assumption}[Greedy $\pi$ Q-V]
For any $(i,h)\in[m]\times[H]$ and function $\oV_{i,h+1}$ and any policy $\pi\in \Pi^{lin}$, we have 
\begin{align*}
\DD_{\delta_a\times \pi_{-i}}\brac{r_{i,h} + \P_h\oV_{i,h+1}}(s) = \phi_i(s,a)^\top \theta^{h,\pi_{-i},\oV}
\end{align*}
for some $\theta^{h,\pi_{-i},\oV}$.
\[\Pi^{lin}:=\left\{\pi_i(\cdot|s) = \arg\max_a \left(\phi(s,a)^\top w^{i}\right)\right\}\]
\end{assumption}

Let us examine each assumption in more detail. For simplicity assume that the MG is layered ($\cS=\cS_1\cup \cdots \cS_H$) so that the $h$ subscript can be dropped.

\paragraph{All $\pi$ V-V.} Fix all other players except $i$. All $\pi$ V-V implies that in $V^\pi_{i}(s) = \phi(s)^\top \theta^{h,\pi}$ for some $\theta^{\pi}$.  Consider two policies $\pi_1$ and $\pi_2$ that differ only by the action taken at $s^*\in\cS_h$. Clearly for $s\neq s^*\in\cS_h$,
\[\phi(s)^\top \left(\theta^{\pi_1}-\theta^{\pi_2}\right)=0.\]
Therefore if $\phi(s^*)\in span(\{\phi(s)\}_{s\neq s^*})$, 
\[\phi(s^*)^\top \left(\theta^{\pi_1}-\theta^{\pi_2}\right)=0.\]
It follows that if $s^*$ is \emph{relevant}, i.e. $\exists$ $\pi_1,\pi_2$ such that $$V^{\pi_1}_h(s^*)\neq V^{\pi_2}_h(s^*),$$
$\phi(s^*)\notin span(\{\phi(s)\}_{s\neq s^*})$. It further follows that all relevant states have linearly independent features, so there can be at most $d$ such states at each layer.

\paragraph{All $\pi$ Q-V.} The argument is very similar to the V-V case. Fix a player $i$ (and drop the subscript for simplicity) and a state $s^*\in \cS_h$. Consider $\pi^1$ and $\pi^2$ that are different only at state $s^*$. By assumption, there exists $\theta^{\pi^1_{-i}}$ such that $\forall s\in\cS_h,a\in\cA_i$
\[\phi(s,a)^\top \theta^{\pi^1} = Q^{\pi^1}(s,a), \quad \phi(s,a)^\top \theta^{\pi^2} = Q^{\pi^2}(s,a).\]
It follows that for every $s\neq s^*\in \cS_h$ and $a\in \cA_i$,
\[\phi(s,a)^\top \left(\theta^{\pi^1_{-i}}-\theta^{\pi^2_{-i}}\right)=0.\]
Therefore if $s^*$ is \emph{not unilateral for player $i$}, e.g. , $\exists$ $a\in\cA_i$ and $\pi, \pi'$ such that
\[Q^\pi(s^*,a)\neq Q^{\pi'}(s^*,a),\]
this action's feature $\phi(s^*,a)$ must be linearly independent from other state-action features. It follows there can be at most $dHm$ non-unilateral states.

%\textbf{Why is such a MG trivial?} 
\yw{Although this looks undesirable at first glance, is such a MG necessarily trivial? For instance, every state in a turned-based MG is unilateral.}

\paragraph{Greedy $\pi$ Q-V} We now argue that the Linear MDP + Tabular MG example actually does NOT satisfy this condition.

To that end, let us first state the example concretely. Let $\cS=\cS^{lin}_1\times \cdots\times \cS^{lin}_m\times \cS^{MG}$, $\cA_i=\cA^{lin}_i\times \cA^{MG}_i$. $\phi(s)$. The linear MDP states and tabular MG states transit independently, i.e. transition is described by
\[P(s^{MG}_{h+1}|s^{MG}_h, a^{MG}_1,\cdots,a^{MG}_m)\]
and 
\[P_i(s^{lin}_{i,h+1}|s^{lin}_{i,h},a^{lin}_{i,h})=\langle \phi_i(s^{lin}_{i,h},a^{lin}_{i,h}), \psi_i(s^{lin}_{i,h+1}) \rangle .\]
Now it remains to choose the feature vector for the combined MG. We consider two possible choices:
\begin{align*}
    \Phi_i(s^{MG},s^{lin}_i,a^{MG}_i,a^{lin}_i) &= [\phi_i(s^{lin}_{i,h},a^{lin}_{i,h}), e(s^{MG},a^{MG_i})] \tag{direct sum}\\
    \Psi_i(s^{MG},s^{lin}_i,a^{MG}_i,a^{lin}_i) &= \phi_i(s^{lin}_{i,h},a^{lin}_{i,h}) \otimes e(s^{MG},a^{MG_i}) \tag{direct product}.
\end{align*}
\textbf{With direct-sum feature:} Consider $m=1$, i.e. single player case. In this case the restriction of policy class is irrelevant \yub{since there is no opponent} and the Greedy $\pi$ Q-V assumption is essentially reduced to the linear MDP assumption. However when $m=1$ this is NOT a linear MDP in the direct-sum feature. To see this, consider \yub{$r_h=0$ and} $\bar{V}_{h+1}(\cdot) = I[\cdot = (t^{MG}, t^{lin})]$. The Q-V assumption requires
\[P(t^{lin}|s^{lin}_{h},a^{lin}_{h})P(t^{MG}|s^{MG}_{h},a^{MG}_{h}) = \langle \phi(s^{lin}_h,a^{lin}_h),\theta\rangle + q(s^{MG}_h,a^{MG}_h) \]
for some $\theta$ and $q(\cdot,\cdot)$ (depending on $t$). Clearly this cannot be satisfied in general (we need to bend a product structure into an addition structure).

To be more concrete, consider two identical tabular MDPs: at state $s_0$, taking action $x$ will go to state $s_x$; taking action $y$ will lead to state $y$. Denote the two copies of the MDP by superscript $^{(1)}$ and $^{(2)}$. The requirement above implies
\[P(s_x^{(1)}|s^{(1)}_0,a^{(1)})P(s_x^{(2)}|s^{(2)}_0,a^{(2)}) = q_1(s^{(1)}_0,a^{(1)}) + q_2(s^{(2)}_0,a^{(2)}).\]
This amounts to decomposing the matrix
\[\left[\begin{matrix}
1&0\\
0&0
\end{matrix}\right] = \left[\begin{matrix}
a&a\\
b&b
\end{matrix}\right] + \left[\begin{matrix}
c&d\\
c&d
\end{matrix}\right],
\]
which clearly is impossible.

\textbf{With direct-product feature:} It seems that using direct-sum feature doesn't capture the factored structure even when $m=1$; it is then natural to consider direct-product feature $\Psi$. At least when $m=1$, we are certain that the MDP is indeed a linear MDP in $\Psi$. 

However the Q-V condition requires more than that. We need for any $V:\cS^{MG}\times \cS^{lin}_i\to [0,H]$,~\yub{$V=V_{h+1}$ can be taken to depend on parts that are only }
\begin{align*}
    &\sum_{a^{MG}_{-i}}\sum_{s^{MG}_{h+1}\in \cS^{MG}}\sum_{s^{lin}_{h+1}\in\cS^{lin}_i} \langle \phi_i(s^{lin}_i,a^{lin}_i), \psi(s^{lin}_{h+1}) \rangle P(s^{MG}_{h+1}|s^{MG}_h,a^{MG}_h,a^{MG}_{-i}) \pi_{-i}(a^{MG}_{-i}|s^{MG}_h,s^{lin}_{1},\cdots,c^{lin}_{m}) V(s_{h+1}^{MG}, s_{i,h+1}^{lin})\\
    =& \langle \phi_i(s^{lin}_i, a^{lin}_i),\theta^{V,\pi_{-i}}\rangle \times Q(s^{MG},a^{MG}_i)
\end{align*}
for some $\theta$ and $Q$. Clearly the problem hinges on whether $a^{MG}_{-i}$ can depend on $s^{lin}_{j}$ ($j\neq i$), since they are absent on the RHS. However, the problem with direct-product features is that (somewhat counter-intuitively) the greedy policies are not factored, and that for greedy policies $\pi^{-i}$ can depend on $s^{lin}_{j}$ ($j\neq i$).

In other words, we are wondering for a $\theta\in\R^{dSA}$, for
\begin{align*}
(a,a')&=\arg\max_{a,a'} \langle \phi(s',a')\otimes e_{s,a}, \theta\rangle\\
&= \arg\max_{a,a'} \langle \phi(s',a'), \theta(s,a,\cdot) \rangle, 
\end{align*}
is $a$ independent of $s'$. This is not true in general; a counter-example is given on Scribble.

\yub{Intuition: greedy policy wrt product feature induces a correlation between $a_i^{lin},a_i^{MG}$?}

\yub{I feel like to product feature is perhaps unnatural (as a solution to make single-agent case satisfy the completeness)... But the counterexample with sum feature says something important. It shows completeness wrt any $V_{h+1}$ (which we previously took for granted and did not discuss in detail) is too strong, essentially makes the problem linear MDP to each player. Even in general, not specific to this particular game, we should think more carefully how strong the completeness thing is.}

\yub{To remedy, can we just assume optimistic closure (not sure how weaker that is though), where the form of the optimistic value in the next layer is some linear + bonus thing, and the linear has to be some $V^\pi$, i.e. true value function of some policy.}

\paragraph{Greedy V-V} It has been argued before that V-V implies Q-V. We should expect the same for linear V-V.

Also, V-V requires actions between states to be ``associated'', which can be regarded as unnatural.

==> notations.tex <==
\usepackage{fullpage}
\usepackage{parskip}
\usepackage{enumitem}
\usepackage{amsmath,amssymb}

\usepackage[round,compress]{natbib}
\usepackage{color}
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amsfonts}
\allowdisplaybreaks

\usepackage{algorithm}
\usepackage[noend]{algorithmic}

\usepackage{url}
\usepackage[breaklinks=true]{hyperref}
\usepackage{breakcites}
\usepackage[usenames,dvipsnames]{xcolor}
\hypersetup{
  colorlinks,
  citecolor=blue!70!black,
  linkcolor=blue!70!black,
  urlcolor=blue!70!black
}


\newcommand{\piout}{\pi^{\rm out}}
\renewcommand{\P}{\mathbb{P}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\I}{\mathbf{I}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Z}{\mathbb{Z}}
\renewcommand{\hat}{\widehat}
\newcommand{\eps}{\varepsilon}
\renewcommand{\epsilon}{\varepsilon}

\renewcommand{\set}[1]{{\left\{ #1 \right\}}}
\newcommand{\abs}[1]{{\left| #1 \right|}}
\newcommand{\paren}[1]{{\left( #1 \right)}}
\newcommand{\brac}[1]{{\left[ #1 \right]}}


\newcommand{\cD}{\mathcal{D}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cI}{\mathcal{I}}


\newcommand{\up}[1]{\overline{ #1}}
\newcommand{\low}[1]{\underline{ #1}}
\newcommand{\alg}{\textsc{Routine}}
\newcommand{\reg}{\textrm{Regret}}
\newcommand{\poly}{{\mathrm{poly}}}
\newcommand{\ellip}{\textrm{Estimate}}
\newcommand{\trans}{^{\rm T}}

\newcommand{\defeq}{\mathrel{\mathop:}=}
\newcommand{\eqdef}{=\mathrel{\mathop:}}

\newtheorem{condition}{Condition}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}[theorem]{Assumption}


\newcommand{\Pim}{\Pi_{\rm DM}}
\newcommand{\Vb}{\up{V}}
\renewcommand{\a}{\mathbf{a}}


\newcommand{\fu}{\up{f}}
\newcommand{\fl}{\low{f}}
\renewcommand{\th}{^{\rm th}}

% Norms for convenience, along with sizes
\newcommand{\norm}[1]{\left\|{#1}\right\|} % A norm with 1 argument
\newcommand{\lone}[1]{\norm{#1}_1} % l1 norm
\newcommand{\ltwo}[1]{\norm{#1}_2} % l2 norm
\newcommand{\linf}[1]{\norm{#1}_\infty} % l-infinity norm
\newcommand{\lzero}[1]{\norm{#1}_0} % l0 norm
\newcommand{\dnorm}[1]{\norm{#1}_*} % Dual norm
\newcommand{\lfro}[1]{\left\|{#1}\right\|_{\sf Fr}} % Frobenius norm
\newcommand{\lnuc}[1]{\left\|{#1}\right\|_*} % Nuclear norm
\newcommand{\matrixnorm}[1]{\left|\!\left|\!\left|{#1}
  \right|\!\right|\!\right|} % Matrix norm with three bars
\newcommand{\opnorm}[1]{\norm{#1}_{\rm op}} % Operator norm with three bars
\newcommand{\normbigg}[1]{\bigg\|{#1}\bigg\|} % A norm with 1 argument and bigg
                                              % brackets.
\newcommand{\normbig}[1]{\big\|{#1}\big\|} % A norm with 1 argument and big
                                           % brackets.
\newcommand{\normBig}[1]{\Big\|{#1}\Big\|} % A norm with 1 argument and Big
                                           % brackets
\newcommand{\lonebigg}[1]{\normbigg{#1}_1} % l1 norm
\newcommand{\ltwobigg}[1]{\normbigg{#1}_2} % l2 norm
\newcommand{\ltwobig}[1]{\normbig{#1}_2} % l2 norm
\newcommand{\ltwoBig}[1]{\normBig{#1}_2} % l2 norm
\newcommand{\linfbigg}[1]{\normbigg{#1}_\infty} % l-infinity norm
\newcommand{\norms}[1]{\|{#1}\|} % A norm with 1 argument and normal (small)
                                 % brackets.
\newcommand{\matrixnorms}[1]{|\!|\!|{#1}|\!|\!|} % Small matrix norm
\newcommand{\matrixnormbigg}[1]{\bigg|\!\bigg|\!\bigg|{#1}\bigg|\!\bigg|\!\bigg|} % Small matrix norm
\newcommand{\lones}[1]{\norms{#1}_1} % l1 norm with small brackets
\newcommand{\ltwos}[1]{\norms{#1}_2} % l2 norm with small brackets
\newcommand{\linfs}[1]{\norms{#1}_\infty} % l-infinity norm with small brackets
\newcommand{\lzeros}[1]{\norms{#1}_0} % l0 norm with small brackets
\newcommand{\lambdamax}[1]{\lambda_{\max}({#1})}
\newcommand{\lambdamin}[1]{\lambda_{\min}({#1})}
\newcommand{\vmax}[1]{v_{\max}({#1})}
\newcommand{\vmin}[1]{v_{\min}({#1})}

\newcommand{\CCEGap}{{\rm CCEGap}}

\newcommand{\lin}{{\rm lin}}
\newcommand{\BR}{{\sf BR}}
\newcommand{\Mar}{{\sf Mar}}

\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\newcommand{\Btheta}{{B_\theta}}
\newcommand{\Bphi}{{B_{\phi}}}

\newcommand{\mc}[1]{\mathcal{#1}}

\newcommand{\wt}{\widetilde}
\newcommand{\wb}{\overline}
\newcommand{\what}{\widehat}
\newcommand{\grad}{\nabla}
\newcommand{\tO}{\wt{\mc{O}}}

\newcommand{\red}[1]{{\color{red} {#1}}}

\newcommand{\indic}[1]{\mathbf{1}\left\{#1\right\}} % Indicator function
\newcommand{\indics}[1]{1\{#1\}} % Indicator function small
% \newcommand{\bindic}[1]{\mathbf{1}\left\{#1\right\}} % Indicator
% function
\newcommand{\<}{\left\langle}
\renewcommand{\>}{\right\rangle}

\newcommand{\Reg}{{\rm Reg}}


\newcommand{\D}{\mathbb{D}}



\newcommand{\visit}{{\rm visit}}
\newcommand{\cov}{{\rm cov}}
\newcommand{\cover}{{\rm cover}}
\newcommand{\est}{{\rm est}}
\newcommand{\Unif}{{\rm Unif}}
\newcommand{\regress}{{\rm reg}}

\newcommand{\Nv}{N_{\rm visit}}
\newcommand{\setto}{\leftarrow}

\newcommand{\Ns}{\widetilde{N}}
\newcommand{\Nb}{\hat{N}}


\newcommand{\oV}{\wb{V}}
\newcommand{\hV}{\hat{V}}
% \newcommand{\cV}{\mathcal{V}}
\newcommand{\opi}{\overline{\pi}}
\newcommand{\hpi}{\hat{\pi}}
\newcommand{\hx}{\hat{x}}
\newcommand{\hy}{\hat{y}}
\newcommand{\tpi}{\tilde{\pi}}
\newcommand{\II}{\mathbb{I}}
\newcommand{\EE}{\mathbb{E}}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\VV}{\mathbb{V}}
\newcommand{\DD}{\mathbb{D}}
\newcommand{\nrm}[1]{\left\|#1\right\|}



\newcommand{\CovSL}{{\Lambda}_{{\rm lazy},h}}
\newcommand{\CovS}{{\Lambda}_{h}}


\newcommand{\betacce}{\beta_{{\rm cce},i,h}}
\newcommand{\betareg}{\beta_{{\rm regress},i,h}}
\newcommand{\thetas}{\theta^{\star}}

